SeFAR: Semi-supervised Fine-grained Action Recognition with Temporal Perturbation and Learning Stabilization

Human action understanding is crucial for the advancement of multimodal systems. While recent developments, driven by powerful large language models (LLMs), aim to be general enough to cover a wide range of categories, they often overlook the need for more specific capabilities. In this work, we address the more challenging task of Fine-grained Action Recognition (FAR), which focuses on detailed semantic labels within shorter temporal duration (e.g., "salto backward tucked with 1 turn"). Given the high costs of annotating fine-grained labels and the substantial data needed for fine-tuning LLMs, we propose to adopt semi-supervised learning (SSL). Our framework, SeFAR, incorporates several innovative designs to tackle these challenges. Specifically, to capture sufficient visual details, we construct Dual-level temporal elements as more effective representations, based on which we design a new strong augmentation strategy for the Teacher-Student learning paradigm through involving moderate temporal perturbation. Furthermore, to handle the high uncertainty within the teacher model's predictions for FAR, we propose the Adaptive Regulation to stabilize the learning process. Experiments show that SeFAR achieves state-of-the-art performance on two FAR datasets, FineGym and FineDiving, across various data scopes. It also outperforms other semi-supervised methods on two classical coarse-grained datasets, UCF101 and HMDB51. Further analysis and ablation studies validate the effectiveness of our designs. Additionally, we show that the features extracted by our SeFAR could largely promote the ability of multimodal foundation models to understand fine-grained and domain-specific semantics.

==> Contents/checklist.tex <==
\section*{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\subsection*{This paper:}

\begin{enumerate}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes)
\end{enumerate}

\subsection*{Does this paper make theoretical contributions? (yes)}

If yes, please complete the list below.

\begin{enumerate}
    \item All assumptions and restrictions are stated clearly and formally. (yes)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes)
    \item Proofs of all novel claims are included. (yes)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes)
    \item Appropriate citations to theoretical tools used are given. (yes)
    \item All theoretical claims are demonstrated empirically to hold. (yes)
    \item All experimental code used to eliminate or disprove claims is included. (yes)
\end{enumerate}

\subsection*{Does this paper rely on one or more datasets? (yes)}

If yes, please complete the list below.

\begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (partial)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)
\end{enumerate}

\subsection*{Does this paper include computational experiments? (yes)}

If yes, please complete the list below.

\begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix. (no)
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (no)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (partial)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (partial)
    \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (partial)
\end{enumerate}


==> Contents/method.tex <==
% Our framework, SeFAR, as demonstrated in Fig.~\ref{fig:pipeline}, is designed for challenging semi-supervised fine-grained action recognition.
% By adopting several marvelous SSL strategies, 
% we propose innovative strategies and make considerable improvements towards this new challenging scene,
% including \textit{Apical-Basal} Dual-compartment Modeling,
% temporal perturbation by \textit{Basal Retrospective},
% as well as the \textit{Adaptive Regulation}.
% % All their points and details can be found in \cref{sec:framework}.


In this section, we present our SeFAR framework designed for challenging Semi-supervised Fine-grained Action Recognition.
The complete pipeline is shown in Fig.~\ref{fig:pipeline}.
% SeFAR consists of three main strategies, including \textit{Apical-Basal} Dual-compartment Modeling, temporal perturbation by \textit{Basal Retrospective}, as well as the \textit{Adaptive Regulation}.
\vspace{-0.3em}
\subsection{Preliminaries}
\label{sec:pre}

Before delving into specific challenges brought by FAR, we first elaborate on basic notations and essential concepts of the Semi-Supervised Learning (SSL) setting, especially those key components of the original FixMatch~\cite{sohn2020fixmatch} method.


\vspace{-0.2em}
\subsubsection{\ding{113} Teacher \textit{vs.} Student Model.}
A line of SSL frameworks adopts the Teacher-Student dual role-playing setting, where the \textit{Teacher} model needs to generate pseudo-labels based on its predictions for the \textit{Student} to learn from.
Instead of directly sharing weights between teacher and student models~\cite{sohn2020fixmatch}, 
We adopt the idea that ``Mean teachers work better"~\cite{tarvainen2017mean}, using an average of consecutive student models to work as the \textit{Teacher}.
Formally, at a given time step, the weights of the \textit{Teacher} model, $\theta_{t}$, undergo optimization processes based on the already updated weights of the \textit{Student} model, $\theta_{s}$, especially as an exponential moving average of the student weights:
\begin{equation} 
\theta_{t}  \longleftarrow \omega \theta_{s} + (1-\omega)\theta_{t}. \label{4} 
\end{equation}
As pointed out in~\cite{xing2023svformer}, such EMA-Teacher is more suitable and stable for SSL action recognition.


%%%%%%%%%%%%%%%%%% Weak Augmentation v.s. Strong Augmentation
\vspace{-0.2em}
\subsubsection{\ding{113} Weak \textit{vs.} Strong Augmentation.}
One core component within FixMatch~\cite{sohn2020fixmatch} is the construction of contrastive data pairs to facilitate consistency regularization.
This involves the incorporation of both strong and weak augmentations, wherein the term \textit{``augmentation"} assumes a connotation more aligned with distortion rather than a straightforward enhancement, contrary to intuition.
% To achieve this, strong and weak augmentations are adopted, where the word \textit{"augmentation"} here is more like a kind of distortion, instead of a positive process as intuition.
Specifically, strong augmentation ($\mathcal{A}_{strong}$) is usually designed to induce significant perturbation to the original data, thereby producing input for the Student Model.
The Teacher model processes weakly augmented ($\mathcal{A}_{weak}$) samples as input, and derives predictions based on these moderately distorted data samples, as demonstrated in the center part of Fig.~\ref{fig:pipeline}


%%%%%%%%%%% Supervised v.s. Unsupervised Learning
\vspace{-0.2em}
\subsubsection{\ding{113} Labeled \textit{vs.} Unlabeled Data.}
Given a dataset with $N$ samples,
in the SSL setting, 
only a small portion of them have annotated labels, denoted by $\{x_{i},y_{i}\}_{i=1}^{\mathcal{B}_l}$.
The left ${\mathcal{B}_{u}}$ samples, are all unlabeled, denoted by $\{x_{j}\}_{j=1}^{\mathcal{B}_{u}}$.
Note that the labeling ratio $\alpha = \frac{\mathcal{B}_l}{N}$ is usually small (e.g., $0.1$).
For the labeled data, the training process is straightforward, just following the classical supervised learning pipeline, minimizing the 
cross-entropy loss between model predictions $Pred(x_i)$ and labels $y_i$:
\begin{equation}  
\mathcal{L}_{sup} = \frac{1}{\mathcal{B}_l}\sum^{\mathcal{B}_l}_{i=1}\mathcal{H}(y_i, Pred(x_i)). \label{eq2} 
\end{equation}  
However, for the unlabeled data $x_j$, there is no label to work as the supervision.
To solve this,
we generate pseudo-labels
from the Teacher model predictions $\mathcal{F}^{T}$, and then 
calculate the unsupervised loss as follows:
\begin{equation}
  \begin{aligned}
\hat{y_j} &= max( {\mathcal{F}}_{t} (\mathcal{A}_{weak}(x_j)),\\
\mathcal{L}_{un} &= \frac{1}{\mathcal{B}_{u}}\sum^{\mathcal{B}_u}_{j=1}\mathbf{1}( \hat{y_j} > \tau)\mathcal{H}(\hat{y_j}, \mathcal{F}_s(\mathcal{A}_{Strong}(x_j))), \label{eq3} 
\end{aligned}  
\end{equation}
where $\tau$ represents the predefined threshold for confidence scores and $\mathbf{1}$ denotes the indicator function.
To summarize, the comprehensive objective function for the whole pipeline encompasses both the supervised and unsupervised loss, weighted by hyperparameters, $\gamma_1$ and $\gamma_2$:
\begin{equation} 
\mathcal{L}= \gamma_{1} \mathcal{L}_{sup} + \gamma_2 \mathcal{L}_{un}. \label{eq4} 
\end{equation} 


\vspace{-0.3em}
\subsection{The SeFAR Framework}
\label{sec:framework}
In this work, we for the first time shed light on the task of Fine-grained Action Recognition (FAR) in the Semi-Supervised Learning (SSL) setting.
This new task brings unprecedented challenges, including but not limited to: 
\ding{182} How to mine abundant and detailed visual information for differentiating subtle differences between fine-grained actions?
\ding{183} How to adapt the original SSL strategies, \textit{e.g.}, consistency regularization to fit the ``temporal-matters" FAR task?
\ding{184} How to deal with the unstable pseudo-labels since the model hesitates between appearance-similar action samples?

To address these, we propose \textbf{SeFAR}, as demonstrated in Fig.~\ref{fig:pipeline}.
SeFAR possesses several delicately designed modules to further emphasize the intrinsic of FAR, including the \textit{Apical-Basal} Dual-compartment Modeling along with the temporal perturbation by \textit{Basal-Retrospective}, and stabilizing learning via \textit{Adaptive Regulation}. We further illustrate the MLLM empowering process with SeFAR.



\vspace{-0.2em}
\subsubsection{Apical-Basal Dual-compartment Modeling.}
% FAR requires distinguishing between subtly different action instances and is recognized to be a more challenging task~\cite{shao2020finegym, xu2022finediving, li2022dynamic, leong2022combined} compared with coarse-grained action recognition.
Distinct from coarse-grained action recognition, in FAR, high similarity is shared in large parts of visual content (\textit{e.g.}, scenes, objects),
making it intractable for models to capture discriminative details effectively. To this end, we draw inspiration from the human brain's neural mechanisms, \textit{i.e.}, the Apical-Basal compartments in L5 cortical pyramidal neurons. Specifically, the \textit{Apical} compartment integrates high-level context or global information, while the \textit{Basal} compartment focuses on specific, localized sensory input. Leveraging this dual-compartment processing strategy, we introduce the Apical-Basal dual-compartment modeling strategy, as depicted in Fig.~\ref{fig:pipeline}.

Specifically, given an action video comprising $N$ frames, 
we first trim it into the $K$ segments following the common paradigm~\cite{wang2016temporal}.
Within each segment, we randomly sample one frame, obtaining a frame sequence $\{f_1, ..., f_K\}$ to represent the video, which different from previous incremental sampling works, \textit{e.g.}, TPN~\cite{yang2020temporal}. 
Inspired by previous action understanding works~\cite{zhou2018temporal,zhao2017temporal} which have shown considerable performance gain using hierarchical temporal aggregation, here we also propose to construct multi-granular visual information package $p_i$ by combining different frames.
Note that the frame aggregation is not random.
For a certain $p_i$, denoted as $P_i$, we first define the temporal length (\textit{i.e.}, L frames), and then perform uniform sampling on $\{f_1, ..., f_K\}$, the sampled frames are then concatenated and encoded by the feature extracting backbone $\mathbf{g}$ (\textit{i.e.}, ViT), obtaining the feature vector $\mathbf{P}_i$. The whole process can be formulated as follows:
\begin{equation}
\begin{aligned}
     p_i &= \{ f_1^{(P_i)}, ..., f_L^{(P_i)}\}, \quad L \leq K, \\
    \mathbf{P}_i &= \mathbf{g} (concat( f_1^{(P_i)}, ..., f_L^{(P_i)} ) ).
\end{aligned}
\end{equation}
The sampling step for $p_i$ could be calculated as $\lfloor \frac{K}{L} \rfloor$.
Theoretically, any integer could be the sampling step.
However, to optimize efficiency, we regulate the sampling frequency and allocate the temporal lengths of the obtained $p_i$ into two distinct levels: Apical and Basal.
% But for efficiency, we control the sampling times and assign the temporal lengths of the obtained $p_i$ to fall into two relative levels :
% global level and local level.
The primary distinction is that the Apical-granularity information packages $p^{(Apical)}$ contain more frames, usually two times more than the longest Basal ones $p^{(Basal)}$.
Once sampled, aggregated, and separately encoded, 
the video sample will be transformed into a set of representative feature vectors $\mathbf{p}_j $.
% $\{ \mathbf{f}_i; \mathbf{p}_j\}$.
% Once sampled and combined, we encode all the originally sampled frames $\{f_1, ..., f_K\}$, as well as the defined frame-wise combinations using the backbone model (\textit{i.e.}, ViT).
% Note that for a specific $p_i$, 
% its feature vector is not just an average of frame-level features,
% but derived through concating input frames to feed into the Backbone.
% its feature vector does not merely constitute an average of frame-level features; rather, it is generated by concatenating input frames before feeding them into the backbone.
All these feature vectors serve as multi-granular visual information carriers, their fused combinations $\mathbf{d}_r$ are also included as additional features. All of them will be fused for the model to produce the final prediction, as shown in Fig.~\ref{fig:pipeline}.
%and will be fused for the model to produce final predictions, \textcolor{red}{as shown in }.
% The effectiveness of such a multi-granular information mining process is verified by Analysis and Studies in \cref{sec:ablation}.


\vspace{-0.2em}
\subsubsection{Temporal Perturbation by Basal-Retrospective.}
Weak-to-strong augmentation for consistency regularization is popularized by FixMatch~\cite{sohn2020fixmatch} in image-based tasks.
However, as pointed out in~\cite{xing2023svformer}, augmentation designed for images is insufficient for video tasks. 
To elaborate,
weakly distorted data are expected to produce supervision for strongly distorted ones, and the key during this process is to make perturbations to the most crucial part of the data that we want the model to attend to~\cite{sohn2020fixmatch, xie2020unsupervised, kurakin2020remixmatch}.
Considering the FAR task, two core insights are emphasized to construct the weak-to-strong pairs:
\ding{172} Temporal matters (\textit{e.g.}, the temporal order and the temporal structure, etc);
\ding{173} The temporal perturbation should not affect the semantic distinctiveness of action categories.

By cooperating with the Apical-Basal dual-compartment modeling strategy, we propose a new strong augmentation operation through the Basal-Retrospective.
In further detail, such augmentation is applied to those information packages $p_i$ rather than individual frames.
For the Apical-level information package $p^{(Apical)}$, the frame order is preserved;
while \textit{all} the remaining Basal-level information packages are \textit{distorted through reversing frames}, as shown in Fig.~\ref{fig:pipeline}.

In formal, assume $M$ information packages are aggregated, resulting in $\{ p_i \}_{i=1}^{M}$, where the one with the most frames, $P_M$, serves as the Apical context, the augmentation process is achieved as follows:
\begin{equation}
    \mathcal{A}_{strong} (\{ p_i \}_{i=1}^{M}) = \{\phi({p}_1), \phi({p}_2), ..., \phi({p}_{M-1}), p_M\}, 
    \label{eq-order}
\end{equation}
where $\phi$ represents reversing frame orders, \textit{e.g.}, from 1,2,3 to 3,2,1.
Our Basal Retrospective strategy introduces moderate temporal perturbation compared with total shuffling,
and it also outperforms previous strategies, \textit{e.g.}, temporal warping~\cite{xing2023svformer}.
Moreover, preserving the temporal order of the Apical package 
ensures the temporal directionality to be inherent in actions (\textit{e.g.}, \textit{``giant circle backward" vs. ``giant circle forward"}, etc.).



\begin{figure}
    \centering
   \includegraphics[width=\linewidth]{stablizing.png}
   \vspace{-1.6em}
    \captionof{figure}{\label{fig:prediction}
    \textbf{Stabilizing Optimization via Adaptive Regulation.} 
    For $K$ unlabeled videos, the Teacher Model predicts each video multiple times to capture the distribution of predictions, which shows less variability on coarse-grained data and more on fine-grained data. An adaptive coefficient $\eta$ is calculated from the mean and variance of the distribution to reduce large fluctuations and stabilize training.
    % For $K$ unlabeled videos, the Teacher Model makes predictions for each video. The predictions exhibit smaller fluctuations on the coarse-grained dataset but larger ones on the fine-grained dataset. Therefore, the Teacher Model needs to predict the same video multiple times to derive the distribution of multiple predictions, and calculate the adaptive coefficient $\eta$ based on the mean and variance of the distribution to mitigate the impact of significant prediction fluctuations and stabilize the training process.
    }
    \vspace{-1em}
\end{figure}
%

\begingroup
\begin{table*}[ht]
\vspace{-0.6em}
  \caption{\textbf{Comparison with state-of-the-art semi-supervised action recognition methods on fine-grained datasets.} We employ SeFAR with a sampling combination of \{2-2-4\}. The primary evaluation metric is top-1 accuracy. In this table, ``V" within ``Input" denotes RGB video, while ``G" represents temporal gradients. ``ImgNet" indicates the utilization of models pre-trained on ImageNet~\cite{russakovsky2015imagenet}, while ``\#F" signifies the number of input frames. The labeling rates of the data are indicated by ``5\%", ``10\%", and ``20\%" in the datasets. The best results are highlighted in \textbf{Bold}, and the second-best \underline{Underlined}.}
  \vspace{-0.6em}
  \setlength{\tabcolsep}{1.5pt} % Default value: 6pt
  \begin{subtable}{\textwidth}
  \renewcommand{\arraystretch}{1}
  \centering
  \small
   \begin{tabular}{lcccccc|cccccc}
     \hlineB{2.5}
     \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\textbf{ImgNet}} & \multirow{2}{*}{\textbf{Params}} & \multirow{2}{*}{\textbf{\#F}} & \multirow{2}{*}{\textbf{Epoch}} & \multicolumn{2}{c}{\textbf{Gym99}} & \multicolumn{2}{c}{\textbf{Gym288}} &\multicolumn{2}{c}{\textbf{Diving}}\\
     \cline{8-13}
     & & & & & & & \textbf{5\%} & \textbf{10\%} & \textbf{5\%} & \textbf{10\%} & \textbf{5\%} & \textbf{10\%}\\
     \hlineB{2}
     MemDPC (ECCV'20)~\cite{han2020memory} &  3D-ResNet-18 & V & \ding{55} & 15.4M & 16 & 500 & 10.8 & 24.1 & 14.5 & 21.3 & 54.3 & 62.0\\
     LTG (CVPR'22)~\cite{xiao2022learning} & 3D-ResNet-18 & VG & \ding{55} & 68.3M & 8 & 180 & 34.3 & 45.8 & 16.2 & 38.7 & 59.8 & 64.3\\
     % TimeBalance (CVPR2023)~\cite{dave2023timebalance} & 3D-ResNet-50 & V & \ding{55} & 250 & 0 & 0 & 0 & 0 & 0 & 0\\
     SVFormer (CVPR'23)~\cite{xing2023svformer} & ViT-B & V & \ding{51} & 121.4M & 8 & 30 & 31.4 & 47.9 & 21.3 & 39.6 & 59.1 & 70.8\\
     \hline
     \rowcolor{cyan!10}
     SeFAR-S (Ours) & VIT-S & V & \ding{51} & 31.2M & 8 & 30 & \underline{36.7}  & \underline{56.3} & \underline{27.8} & \underline{46.9} & \underline{72.2} & \underline{78.4} \\
     \rowcolor{cyan!10}
     SeFAR-B (Ours) & VIT-B & V & \ding{51} & 122.1M & 8 & 30 & \textbf{39.0}  & \textbf{56.9} & \textbf{28.3} & \textbf{48.1} & \textbf{72.8} & \textbf{80.9} \\
     \hlineB{2.5}
   \end{tabular}
   \caption{Results of elements across all events.}
   \label{tab:sub1.1}
   \end{subtable}
   \hfill
   % \vspace{-0.4em}
   \setlength{\tabcolsep}{5.9pt}
    \begin{subtable}{0.5\linewidth}
    \renewcommand{\arraystretch}{1}
    \centering
    \small
    \begin{tabular}{lcccccc}
     \hlineB{2.5}
     \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{UB}} & \multicolumn{2}{c}{\textbf{FX}} & \multicolumn{2}{c}{\textbf{10m}}\\
     \cline{2-7}
     & \textbf{10\%} & \textbf{20\%} & \textbf{10\%} & \textbf{20\%} & \textbf{10\%} & \textbf{20\%}\\
     \hlineB{2}
     MemDPC & 20.7 & 19.1 & 13.8  & 15.9 & 65.4 & 71.2\\
     % TCL~\cite{singh2021semisupervised} & 0 & 0 & 0 & 0 & 0 & 0\\
     LTG & 50.5 & 60.5 & 19.6 & 21.6 & 75.2 & 83.5\\
     % TimeBalance~\cite{dave2023timebalance} & 0 & 0 & 0 & 0 & 0 & 0\\
     SVFormer & 52.9 & 66.8 & 20.1 & 28.8 & 73.8 & 85.9\\
     \hline
     \rowcolor{cyan!10}
     SeFAR-S (Ours) & \underline{56.9} & \underline{73.8}& \underline{23.8} & \underline{42.9} & \underline{85.5} & \underline{94.0}\\
     \rowcolor{cyan!10}
     SeFAR-B (Ours) & \textbf{58.5} & \textbf{75.5}& \textbf{27.6} & \textbf{44.2} & \textbf{87.4} & \textbf{94.6}\\
     \hlineB{2.5}
   \end{tabular}
   \caption{Results of elements within an event.}
   \label{tab:sub1.2}
   \end{subtable}
   \hfill
   \setlength{\tabcolsep}{5.8pt}
    \begin{subtable}{0.5\linewidth}
    \renewcommand{\arraystretch}{1}
    % \centering
    \small
    \begin{tabular}{lcccccc}
     \hlineB{2.5}
     \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{UB-S1}} & \multicolumn{2}{c}{\textbf{FX-S1}} & \multicolumn{2}{c}{\textbf{5253B}}\\
     \cline{2-7}
     & \textbf{10\%} & \textbf{20\%} & \textbf{10\%} & \textbf{20\%} & \textbf{10\%} & \textbf{20\%}\\
     \hlineB{2}
     MemDPC & 17.2 & 21.1 & 15.4 & 20.1 & 82.2 & 89.5\\
     % TCL~\cite{singh2021semisupervised} & 32.6 & 0 & 0 & 0 & 0 & 0\\
     LTG & 21.3 & 29.7 & 14.6 & 19.3 & 64.6 & 76.9\\
     % TimeBalance~\cite{dave2023timebalance} & 0 & 0 & 0 & 0 & 0 & 0\\
     SVFormer & 28.9 & 47.3 & 18.8 & 22.5 & 86.6 & 90.1\\
     \hline
     \rowcolor{cyan!10}
     SeFAR-S (Ours) & \underline{36.6} & \underline{55.3} & \underline{19.2} & \underline{25.5} & \underline{96.4} & \underline{97.3} \\
     \rowcolor{cyan!10}
     SeFAR-B (Ours) & \textbf{37.1} & \textbf{56.8} & \textbf{20.1} & \textbf{26.5} & \textbf{97.0} & \textbf{97.8} \\
     \hlineB{2.5}
   \end{tabular}
   \caption{Results of elements within a set.}
   \label{tab:sub1.3}
   \end{subtable}
   \label{tab:1}
   \vspace{-1.4em}
\end{table*}
\endgroup


\vspace{-0.2em}
\subsubsection{Stabilizing Optimization via Adaptive Regulation.}
As mentioned, due to the challenging intrinsic of FAR,
models usually swayed precariously between categories with subtle differences~\cite{shao2020finegym}.
During experiments, the greater the uncertainty of the model's predictions, the less reliable the model's predictions are.
Such unstable predictions of the teacher model will result in ambivalent and invalid pseudo-labels for the student,
making the whole learning process suffer.

To solve this,
we first let the \textit{teacher} model generate predictions $U$ times ($U$ is set to 10 in experiments) for a given unlabeled video, and these predictions may vary largely.
Then, based on these, we calculate the mean prediction confidence and standard deviation for each category.
For the $i^{th}$ prediction, the predicted probability across all categories constitutes a probability distribution. From this distribution, we can obtain the maximum prediction confidence value $\mu^{i}$ and calculate its standard deviation $\sigma^{i}$.
We select the highest confidence value $\mu^* = max(\mu^{i})$,
along with its corresponding standard deviation $\sigma^*$, as shown in Fig.~\ref{fig:prediction}.

Based on such $\mu^*$ and $\sigma^*$,
we propose to calculate the dynamic coefficients $\tau_1$ and $\tau_2$ to obtain $\eta$, which is further used for adjusting losses derived from unlabeled data samples:
\begin{equation}
  \begin{aligned}
\tau_1 & =  sigmoid(e^{\mu^*} - e), \\
\tau_2 & = (sigmoid(\frac{1}{\beta\sigma^*+\epsilon})-0.5),
\end{aligned}  
\end{equation}
\noindent where $\beta$ is related to the model dropout and $\epsilon$ is a steady parameter.
To elaborate,
$\tau_1$ will increase rapidly as $\mu^*$ increases, which enhances high-confidence predictions,
while on the other hand, $\tau_2$ suppresses the unstable predictions (\textit{i.e.}, with high standard deviation $\sigma$).
The obtained adaptive coefficient $\eta = \tau_1 \cdot \tau_2,$ is more flexible and beneficial than a predefined hyperparameter. 
Additionally, for unlabeled data, we also adopt the mixing strategy as in SVFormer~\cite{xing2023svformer}, where the mixture of two unlabeled samples, $\lambda x_1  + (1-\lambda)x_2$, could also serve as input, and the supervision is correspondingly obtained as a mixed version (Details could be found in~\cite{xing2023svformer}).
Here for adjusting $\mathcal{L}_{mix}$, we achieve its coefficient in a similar mixed manner, denoted by $\eta^{'}=\lambda\eta_{1}+(1-\lambda)\eta_{2}$, where $\eta_{1}, \eta_{2}$ are individually calculated based on $x_1$ and $x_2$. 
Finally, the total loss of the whole FARmatch framework is as follows:
\begin{equation}
\mathcal{L} = \mathcal{L}_{sup} + \xi(\eta\mathcal{L}_{un} + 
 \eta^{'} \mathcal{L}_{mix}),
 \label{eq-loss} 
\end{equation}
where $\xi = sin(\frac{n}{M_n})$ is a warmup coefficient calculated using the current epoch number $n$ and the max epoch $M_n$.



\vspace{-0.2em}
\subsubsection{SeFAR Empowering MLLM.}
As illustrated in Fig.~\ref{fig:finegrained}, recent advanced MLLMs exhibit suboptimal performance on the FAR task. This is largely due to the intricate and highly variable temporal features inherent in fine-grained actions. However, addressing this issue through conventional approaches (\textit{e.g.}, fine-tuning) reintroduces challenges related to high-quality data collection and annotation, and also leads to increased computational costs. Given that SeFAR, as introduced earlier in this section, is designed to be effective in semi-supervised scenarios (\textit{i.e.}, low-labeling environments), we pose the question: \textit{``Is developing such data-reliant weak, and more specific frameworks necessary for fine-grained visual understanding?"}

The answer is yes supported by the results in Tab.~\ref{tab:mllm}. 
Following the common MLLM paradigm, a frozen visual encoder is paired with a LLM. This combination enables multimodal capabilities by aligning visual and textual features through an adaptor (\textit{e.g.}, Q-Former~\cite{li2023blip}). Specifically, as shown in Fig.~\ref{fig:pipeline}, the features produced by SeFAR are first mapped through a fully connected layer and then fed into the Q-Former, which aligns the input video features with the textual space. These aligned features are subsequently concatenated with the text embeddings and passed into the LLM to generate the corresponding answers.

% 被众多的MLLM采用的BLIP-2框架使用冻结的视觉编码器与LLM，通过一个轻量化的转换结构Q-Former进行视觉与文本特征的对齐，赋予LLM多模态能力。受BLIP-2框架的启发，我们可以替换任一的冻结的视觉编码器，在相同数据集上训练Q-Former，以比较不同视觉编码器对MLLM性能的影响。

% So that we can significantly improve the performance of MLLMs on the FAR task by substituting ViT features with those from SeFAR. We leverage the Q-former in \cite{li2023blip} to enhance the performance of MLLMs on the FAR-QA task. As depicted in Figure 2, the features output by SeFAR are mapped through a fully connected layer and fed into the Q-former. The Q-former then aligns the input video features with the text space. Ultimately, these features are concatenated with the text embeddings from the LLM and fed into the LLM to generate corresponding answers.

